ReFeree: Radar-Based Lightweight and Robust Localization using Feature and Free space

Place recognition plays an important role in achieving robust long-term autonomy. Real-world robots face a wide range of weather conditions (e.g. overcast, heavy rain, and snowing) and most sensors (i.e. camera, LiDAR) essentially functioning within or near-visible electromagnetic waves are sensitive to adverse weather conditions, making reliable localization difficult. In contrast, radar is gaining traction due to long electromagnetic waves, which are less affected by environmental changes and weather independence. In this work, we propose a radar-based lightweight and robust place recognition. We achieve rotational invariance and lightweight by selecting a one-dimensional ring-shaped description and robustness by mitigating the impact of false detection utilizing opposite noise characteristics between free space and feature. In addition, the initial heading can be estimated, which can assist in building a SLAM pipeline that combines odometry and registration, which takes into account onboard computing. The proposed method was tested for rigorous validation across various scenarios (i.e. single session, multi-session, and different weather conditions). In particular, we validate our descriptor achieving reliable place recognition performance through the results of extreme environments that lacked structural information such as an OORD dataset.

==> background.tex <==
\section{Background}
Radar image's intensity, which is the reflection coefficient of the target, is proportional to the Radar Cross Section (RCS) value.
RCS is the ratio of the reflected power to the incident power density, meaning that higher RCS values correspond to more power being reflected to the radar. 
RCS is determined by factors such as the size of the target, shape, material, polarization, and frequency of the incident wave, as well as the incidence and reflection angles of the target.
Intuitively, larger sizes result in larger RCS values.
Additionally, the shape of the target is crucial; if it is designed to scatter waves, the RCS decreases.
The material also plays a significant role; materials such as wood or plastic exhibit lower reflection, resulting in smaller RCS values, whereas metallic objects have higher RCS values.
Unfortunately, multipath and noise are potentially high values, which can overshadow meaningful information. 

==> method.tex <==
% ==============================================================================================
\begin{figure*}[t]
	\centering
	\def\width{0.98\textwidth}%
    {%
        \includegraphics[clip, trim= 0 173 0 118, width=\width]{figs/pipeline/pipeline.pdf}
    }
        \caption{Our method's pipeline. } 
% \vspace{-0.5cm}
\label{fig:pipeline}
\end{figure*}
% ==============================================================================================

\section{Method}
\ac{Radar} image's intensity is heavily related to RCS, it is proportional to the latent power multiplied by the RCS of the target \cite{harlow2023new}.
Radar image define $\mathcal{I} \in\mathbb{R}^{\mathcal{H} \times \mathcal{W}}$ in polar coordinates, where $\mathcal{H}$ and $\mathcal{W}$ are the image's height and width, respectively.
The dimensions $\mathcal{H}$ and $\mathcal{W}$ are associated with range and angle, and encapsulating semi-metric information.
In this section, we describe the process of creating our \textit{ReFeree} from the \ac{Radar} image $\mathcal{I}$, recognizing revisited places by comparing two \textit{ReFerees}, estimating the initial guess, and optimizing the pose graph as shown in \figref{fig:pipeline}.
 
\subsection{Place Recognition}
\subsubsection{Feature Extraction}
As mentioned earlier, materials such as wood or plastic frequently exhibit smaller RCS values than noise or multipath effects.
Therefore, it is crucial to effectively distinguish these meaningful targets from noise or multipath interference and successfully extract them as features.
When extracting features from \ac{Radar} images, using inherently vision-based methods (e.g. SIFT \cite{lowe1999object} or ORB~\cite{rublee2011orb}) makes it difficult to address the noise or multipath as signal processing solutions.
Therefore, we select an algorithm designed to process the signals inherent in \ac{Radar} images to extract features \cite{cen2018precise}.
This approach involves decomposing the signal into high or low-frequency signals, integrating them according to a Gaussian scaling factor, and thresholding to extract valid features from the raw \ac{Radar} signal.
By using this method, we reduce noise from the signal and get higher clarity in classifying areas whether detected objects or vacancy. 
% These algorithms are the same as \cite{cen2018precise, cen2019radar}, so please refer to them for details.
We define feature extractor function and feature extracted \ac{Radar} image, as $\phi$ and $\mathcal{I}^{\mathcal{F}}$ respectively, and can be denoted as follows:
\begin{equation}
    \mathcal{I}^{\mathcal{F}} = \phi(\mathcal{I}) 
    \label{equation:spherical_coordinates}, \quad \mathcal{I}^\mathcal{F} \in\mathbb{R}^{\mathcal{H} \times \mathcal{W}}.
\end{equation}

\subsubsection{Free Space Counter}
Inspired by \cite{maffei2020global}, this work proposes a descriptor based on the vacant area (i.e. free space) in $\mathcal{I}^\mathcal{F}$.
Although feature extraction reduces noise and leaves only the relatively robust intensity, the features of \ac{Radar} sensors still have poor resolution, compared to denser sensors such as LiDAR.
Also, noise can have a significant impact due to the nature of \ac{Radar} images, where the number of features is limited. 
Whereas, in free space, noise occupies a relatively smaller proportion compared to features. 
Furthermore, the descriptor matching based on the overlap between free spaces is robust to the noisy and poor resolution characteristics of the \ac{Radar} due to its conciseness.
By improving the methodology of \cite{maffei2020global} and embedding it as a high-dimensional vector, we reorganize it into a suitable representation for \ac{Radar}-based \ac{PR}.
Therefore, we identify free space as:
\begin{equation}
    \psi(\mathcal{T}) = 
    \begin{cases}
        1, & \mbox{if }\mathcal{T}\mbox{ is a \textit{free-space}} \\
        0, & \mbox{otherwise},
    \end{cases}
    \label{equ:free or not}
\end{equation}
where $\mathcal{T} \in \mathbb{R}^2$ is a temporal space.

\noindent As shown in \figref{fig:detailed}, we specify each region using a sliding window approach and count the free space within the window area as follows:
\begin{equation}
	\label{equ:hat_r_referee}
    \mathcal{R}_{[\mathbf{n}_{w}]} = \sum_{j=\alpha*\mathcal{N}_{w}}^{\alpha*(\mathcal{N}_{w}+1)} \left( \sum_{i=1}^{\mathcal{W}} \psi(\mathcal{I}^{\mathcal{F}}_{ji}) \right), \quad \mathcal{R} \in\mathbb{R}^{\mathcal{N}_{w}},
\end{equation}

\begin{equation}
    \label{equ:hat_a_referee}
    \mathcal{A}_{[\mathbf{n}_{h}]} = \sum_{i=\beta*\mathcal{N}_{h}}^{\beta*(\mathcal{N}_{h}+1)}	\left( \sum_{j=1}^{r_i} \psi(\mathcal{I}^{\mathcal{F}}_{ji}) \right), \quad \mathcal{A} \in\mathbb{R}^{\mathcal{N}_{h}},
\end{equation}
% N_w = H/a, N_h = W/beta, 
\noindent where $\alpha, \beta$ is ratio of how much range or angle to contain, $\mathbf{n}_{w}=[1, 2, ..., \mathcal{N}_{w}]$, $\mathbf{n}_{h}=[1, 2, ..., \mathcal{N}_{h}]$, $\mathcal{N}_{w}=\frac{\mathcal{H}}{\alpha}$, and $\mathcal{N}_{h}=\frac{\mathcal{W}}{\beta}$.
The notation $r_i$ is element of farthest feature index vector $\mathcal{V}=[r_1,\cdots,r_\mathcal{W}]$, and it is matched with each col of $\mathcal{I}^{\mathcal{F}}$.

% ==============================================================================================
% \vspace{-0.6cm}
\begin{figure}[h]
	\centering
	\def\width{0.49\textwidth}%
    {%
        \includegraphics[clip, trim= 160 115 190 170, width=\width]{figs/freespace/freespace.pdf}
    }
        % \vspace{-0.5cm}
        \caption{The overview of a free space counter.
                 Function $\psi$ determines the presence of free space within the respective area which is a sliding window consisting of ranges and angles.}	
% \vspace{-0.6cm}
\label{fig:detailed}
\end{figure}
% ==============================================================================================

\subsubsection{ReFeree}
Using the features and the free space, we propose a \ac{Radar}-based efficient global descriptor called \textit{ReFeree}.
Free space can distinguish different spaces on its own, but we count the number of features and use them as weights by composing them into a vector as follows:
\begin{equation}
    \nu(\mathcal{T}) = \mbox{ \# of \textit{features}},
    \label{equ:free or not}
\end{equation}
\begin{equation}
	\label{equ:hat_r_referee}
    \mathcal{R}_{f[\mathbf{n}_{w}]} = \sum_{j=\alpha*\mathcal{N}_{w}}^{\alpha*(\mathcal{N}_{w}+1)} \left( \sum_{i=1}^{\mathcal{W}} \nu(\mathcal{I}^{\mathcal{F}}_{ji}) \right), \quad \mathcal{R}_{f} \in\mathbb{R}^{\mathcal{N}_{w}},
\end{equation}
Since free space and features have an inverse relationship, we create an \textit{R}-\textit{ReFeree} $\hat{\mathcal{R}}$ operated by taking the reciprocal as:
\begin{equation}
	\label{equ:r_referee}
    \hat{\mathcal{R}} = \mathcal{R}_{f} \times \frac{1}{\mathcal{R}}.
\end{equation}
Additionally, since the \textit{A}-\textit{ReFeree} $\hat{\mathcal{A}}$ for initial estimation performs well in finding initial values, we only conduct a normalization to generate the final description as follows:
\begin{equation}
	\label{equ:a_referee}
    \hat{\mathcal{A}} =\frac{\mathcal{A}}{\mathcal{N}_{h} \times \mathcal{W}}.
\end{equation}

\subsubsection{Place Recognition}
We create the \textit{R}-\textit{ReFeree} and recognize revisited places to correct accumulated pose errors. 
We construct a KD-Tree from the candidates to facilitate faster searching, and the distance between the query \textit{R}-\textit{ReFeree} $\hat{\mathcal{R}}^q$ and the candidate \textit{R}-\textit{ReFeree} $\hat{\mathcal{R}}^c$ is calculated using the L2-norm as follows:
\begin{equation}
    \sigma(\hat{\mathcal{R}}^q, \hat{\mathcal{R}}^c) = {||\hat{\mathcal{R}}^q - \hat{\mathcal{R}}^c||} .
    \label{equation:initial_index}
\end{equation}

\subsubsection{Initial Guess}
We can recognize revisited places through the \textit{R}-\textit{ReFeree}, and obtain the initial guess of the two places through the \textit{A}-\textit{ReFeree}. 
Due to the rotational equivalence and semi-metric information of the \textit{A}-\textit{ReFeree}, shifting candidates implies that the index of the closest distance represents $\hat{n}$ as a 1-DoF heading following:
\begin{equation}
    \hat{n} = \argmin\limits_{n \in [\mathbf{n}_{h}]}({||\hat{\mathcal{A}}^q - \hat{\mathcal{A}}^{c}_{n}}||) .
    \label{equation:initial_index}
\end{equation}

\subsection{Loop Closure}
\subsubsection{Odometry}
% 우리는 full SLAM pipeline을 완성하기 위해 Odometry Algorithm을 통합합니다.
% 특히, 우리는 Description에 활용하였던 features를 버리지 않고, Odometry 추정에 사용합니다.
% 하지만, Background figure와 같이 sing radar image의 features는 롤링 셔터와 비슷하게 time dealy가 발생하며, target의 속도에 따라 doppler distortion이 발생합니다.
We are integrating the odometry algorithm called Motion Compensated (MC)-RANSAC \cite{burnett_ral21} to build the full SLAM pipeline.
In particular, we use the features utilized in the description without discarding them and incorporating them into the odometry estimation. 
However, features from the single \ac{Radar} image as represented in \figref{fig:doppler}, experience a time delay similar to a rolling shutter.
By this assumption, it is not allocated to a single timestamp to a single \ac{Radar} image, but it is allocated to each feature of the \ac{Radar} image.
Each feature pair of $M$ match pairs, that result from data association, has time interval $\Delta t_m=\Delta t_{m,2}-\Delta t_{m,1}, (m=1,\cdots,M)$, where $t_{m,1}$ and $t_{m,2}$ is feature timestamp of previous and current radar scan, respectively.
MC-RANSAC estimates constant velocity vector $\varpi=[v,w]$ between $t_{m,1}$ and $t_{m,2}$.
The reason is that estimating $\varpi=[v,w]$ instead of the relative pose is a necessity for considering the possibility of individual measurement times of each feature.
The model of MC-RANSAC is optimized on tangent space that represents lie algebra for relaxing constraints and securing the stability of lie group operation.
Additionally, MC-RANSAC combines Doppler correction to the optimization as \equref{equ:doppler}, \equref{equ:doppler1}.
% 이렇게 해서 얻을 수 있는 이득
% \begin{equation}
% \begin{aligned}
% \zeta({\mathbf{z}}_{t}, {\mathbf{z}}_{t+1})
% \end{aligned}
% \end{equation}

\subsubsection{Registration \& Geometry Verification}
We identify revisited places through the \textit{R}-\textit{ReFeree} and also estimate the initial guess between these revisited places via \textit{A}-\textit{ReFeree}. 
Subsequently, we require a registration process to correct errors in the accumulated map using odometry. 
Therefore, we adopt Nano-GICP \cite{chen2022direct}, which combines the fast speed of Fast-GICP \cite{koide2021voxelized} and the efficient construction of KD-Tree using the open-source library NanoFLANN \cite{blanco2014nanoflann}, not only for registration but also for onboard computing. 
First, we convert the estimated initial guess into a rotation matrix at loop $\mathcal{L}$:
\begin{equation}
 T^{\mathcal{L}}_{k} = \begin{bmatrix}
                  cos\left( \hat{n} \times \frac{360}{\mathcal{N}_{h}} \right) & -sin\left( \hat{n} \times \frac{360}{\mathcal{N}_{h}} \right) \\ 
                  sin\left( \hat{n} \times \frac{360}{\mathcal{N}_{h}} \right) &  cos\left( \hat{n} \times \frac{360}{\mathcal{N}_{h}} \right)
              \end{bmatrix} .	
\end{equation}
Second, we perform scan-to-scan matching between the source point $\mathcal{P}^{s}_{k}$ and the target point $\mathcal{P}^{t}_{k}$ to compute the optimal relative transform as follows:
\begin{equation}
\hat{T}^{\mathcal{L}}_{k} = \argmin\limits_{T^{\mathcal{L}}_{k}}\xi\left( T^{\mathcal{L}}_{k}\mathcal{P}^{t}_{k},\mathcal{P}^{s}_{k} \right).
\end{equation}
The residual error $\xi$ from GICP is defined as:
\begin{equation}
\xi(T^{\mathcal{L}}_{k}\mathcal{P}^{t}_{k},\mathcal{P}^{s}_{k}) = \sum\limits_{i}^{N}d_{i}^{\top}\left( \mathcal{C}^{t}_{k, i} + T^{\mathcal{L}}_{k} \mathcal{C}^{s}_{k, i} T^{\mathcal{L}^{\top}}_{k} \right)^{-1} d_{i} .
\end{equation}
Finally, we obtain the optimal relative transformation through the following optimization function:
\begin{equation}
\hat{T}^{\mathcal{L}}_{k} = \sum\limits_{i}^{N}d_{i}^{\top}\left( \mathcal{C}^{t}_{k, i} + T^{\mathcal{L}}_{k} \mathcal{C}^{s}_{k, i} T^{\mathcal{L}^{\top}}_{k} \right)^{-1} d_{i},
\end{equation}
where $\mathcal{C}^{s}_{k}$ and $\mathcal{C}^{t}_{k}$ are the corresponding estimated covariance matrices associated with each point $i$ of source or target points, and $d_{i} = p_{i}^{t} - T^{\mathcal{L}}_{k}p_{i}^{s}$, $p_{i}^{t} \in \mathcal{P}^{t}_{k}$, $p_{i}^{s} \in \mathcal{P}^{s}_{k}$ for number of corresponding points between $\mathcal{P}^{t}_{k}$ and $\mathcal{P}^{s}_{k}$.

However, even if revisited and current places are in similar positions, mismatches in registration can introduce errors into the map.
Therefore, we progress a geometry verification process by calculating the fitness score through the \ac{ICP} result, which enables us to validate the accurate loop once more as:
\begin{equation}
\varrho(\hat{T}^{\mathcal{L}}_{k}\mathcal{P}^{t}_{k},\mathcal{P}^{s}_{k}) = \frac{1}{N}\sum\limits_{i=1}^{N}||\mathcal{P}^{s}_{k, i} - \hat{T}^{L}_{k}\mathcal{P}^{t}_{k, i}||^2.
\end{equation}

\subsubsection{Pose Graph Optimization}
As pose graph $\mathbf{X}$ from \ac{Radar} odometry contains its accumulated errors due to sensor measurement, loop closing is essential to build a consistent map.
The pose graph optimization of the map is represented as:
\begin{equation}
\begin{aligned}
\hat{\mathbf{X}}=\underset{\mathbf{X}}{\operatorname{argmin}} & \sum \varphi(\mathbf{X}) .
\end{aligned}
\end{equation}
Also, pose graph optimization fuction $\varphi(\cdot)$ is defined as:
\begin{equation}
\begin{aligned}
\varphi(\mathbf{X})= & \sum_t\left\|f\left(\mathbf{x}_t, \mathbf{x}_{t+1}\right)- \zeta({\mathbf{z}}_{t}, {\mathbf{z}}_{t+1})\right\|_{\sum_t}^2 \\
& +\sum_{\langle s, t \rangle \in \mathbb{L}} \left\|f\left(\mathbf{x}_s, \mathbf{x}_t\right)-\xi(\mathcal{P}^{s}_{k},\mathcal{P}^{t}_{k}) \right\|_{\sum_{s, t}}^2,
\end{aligned}
\end{equation}
where $f(\cdot, \cdot)$ is 6-DoF relative pose estimator, $\zeta(\cdot, \cdot)$ is \ac{Radar} odometry estimator with features $z_t$ that contain timestamp, $\xi(\cdot, \cdot)$ is pose aligner between $\mathcal{P}^{t}_{k}$ and $\mathcal{P}^{s}_{k}$ captured in $\mathcal{L} \in \mathbb{L}$. 


==> method2.tex <==
\section{Method}
Radar image define $\mathcal{I} \in\mathbb{R}^{\mathcal{H} \times \mathcal{W}}$ in polar coordinates, where $\mathcal{H}$ and $\mathcal{W}$ are the image's height and width, respectively.
The dimensions $\mathcal{H}$ and $\mathcal{W}$ are associated with range and angle, encapsulating semi-metric information.
In this section, we describe the process of creating the \textit{ReFeree} from the radar image $\mathcal{I}$, recognizing revisited places by comparing two \textit{ReFerees}, and estimating the initial guess.
Also, our method integrates odometry and registration, enabling SLAM, and the results will be discussed in Section~\uppercase\expandafter{\romannumeral4}-G.

\subsubsection{Feature Extraction}
Radar images exhibit a variety of noise characteristics across the sensor range, including spurious returns, complex speckle noise, and multipath reflections where multiple signals are returned from the same object.
To extract meaningful information from noisy data, we use a feature extraction algorithm from \cite{cen2018precise}.
The algorithm involves decomposing the signal into high and low-frequency signals and integrating them according to a gaussian scaling factor.
Finally, the integrated signal goes through the thresholding process to extract valid features from the raw radar signal.
We replace the nonlinear gaussian filter with a linear uniform filter for the time efficiency and versatility of the onboard computer.

\subsubsection{Descriptor Generation based on Free space}
\hl{The noise consists of false positives and false negatives from the feature extractor, and it applies equally to both features and free space.}
% 압축 조금만 더 풀기
If only the features are considered to generate descriptor, the impact of noise is relatively higher than the case of free space.
On the other hand, the descriptor creation based on the free space is robust to the radar's noisy and poor resolution due to its conciseness and relative abundance compared to its features.
By improving the methodology of \cite{maffei2020global} and embedding it as a high-dimensional vector, we reorganize it into a suitable representation for radar-based place recognition.
First, we denote free space identifier as:
\begin{equation}
    \psi(\mathrm{p}) = 
    \begin{cases}
        1, & \mbox{if }\mathrm{p}\mbox{ is a \textit{free-space}} \\
        0, & \mbox{otherwise},
    \end{cases}
    \label{equ:free or not}
\end{equation}
where $\mathrm{p}$ is a pixel value of radar image $\mathcal{I}^{\mathcal{F}}$.
% Second, we count the free space's number in each radar block by utilizing free space counter $\psi$ as follows:
% \begin{equation}
% 	\label{equ:hat_r_referee}
%     \mathcal{R}_{[\mathbf{n}_{w}]} = \sum_{j=\alpha*\mathcal{N}_{h}}^{\alpha*(\mathcal{N}_{h}+1)} \left( \sum_{i=1}^{\mathcal{W}} \psi(\mathcal{I}^{\mathcal{F}}_{ji}) \right), \quad \mathcal{R} \in\mathbb{R}^{\mathcal{N}_{w}},
% \end{equation}

% \begin{equation}
%     \label{equ:hat_a_referee}
%     \mathcal{A}_{[\mathbf{n}_{h}]} = \sum_{i=\beta*\mathcal{N}_{h}}^{\beta*(\mathcal{N}_{h}+1)}	\left( \sum_{j=1}^{r_i} \psi(\mathcal{I}^{\mathcal{F}}_{ji}) \right), \quad \mathcal{A} \in\mathbb{R}^{\mathcal{N}_{h}},
% \end{equation}
Second, we count the free space's number in each radar block by utilizing free space counter $\psi$ as follows:
\begin{equation}
	\label{equ:hat_r_referee}
    \mathcal{R}_{[\mathbf{n}_{w}]}^{f} = \sum_{j=\beta*[\mathbf{n}_{w}]}^{\beta*([\mathbf{n}_{w}]+1)} \left( \sum_{i=1}^{\mathcal{H}} \psi(\mathcal{I}^{\mathcal{F}}_{ij}) \right), \quad \mathcal{R}^{f} \in\mathbb{R}^{\mathcal{N}_{w}},
\end{equation}

\begin{equation}
    \label{equ:hat_a_referee}
    \mathcal{A}_{[\mathbf{n}_{h}]}^{f} = \sum_{i=\alpha*[\mathbf{n}_{h}]}^{\alpha*([\mathbf{n}_{h}]+1)}	\left( \sum_{j=1}^{r_i} \psi(\mathcal{I}^{\mathcal{F}}_{ij}) \right), \quad \mathcal{A}^{f} \in\mathbb{R}^{\mathcal{N}_{h}},
\end{equation}
% N_w = H/a, N_h = W/beta, 
\noindent where $\alpha, \beta$ are how much angle and range each block is containing.
The $\mathbf{n}_{h}=[1, 2, ..., \mathcal{N}_{h}]$ and $\mathbf{n}_{w}=[1, 2, ..., \mathcal{N}_{w}]$, where $\mathcal{N}_{h}=\frac{\mathcal{H}}{\alpha}$, and $\mathcal{N}_{w}=\frac{\mathcal{W}}{\beta}$, are descriptor index vectors and $[\mathbf{n}]$ means each element of $\mathbf{n}_{h}$ or $\mathbf{n}_{w}$.
The notation $r_i$ is element of farthest feature index vector $\bold{R}=[r_1,\cdots,r_\mathcal{H}]$, and it is matched with each column of $\mathcal{I}^{\mathcal{F}}$.

% \subsubsection{ReFeree}
% Using the number of free spaces, we can create a radar based efficient global descriptor.
% However, the number of extracted features is also meaningful, so we don't waste them and use them as weight vectors to create robust descriptors.
% 블럭 내의 information 중요도를 고려하였을 때, free space보다는 feature가 
% 디스크립터에 신호적으로 의미 있는 정보를 통합하기 위해, 우리는 각 블럭의 feature 수를 free space의 수에 대한 가중치로서 사용한다.
% To integrate signal-related meaningful information into the descriptor, we utilize the number of features in each block, weighted by the amount of free space.
% radar image의 feature가 신호 처리 분야적인 측면에서 의미있는 정보를 담고 있으므로, 우리는 각 블럭의 feature 수를 free space의 수에 대한 가중치로서 사용한다.
As the features of a radar image contain meaningful information from a signal processing perspective, we utilize the number of features in each block as a weight for the amount of free space.
To generate the weight vector, we denote feature identifier $\nu$ as:
\begin{equation}
    \nu(\mathrm{p}) = 
    \begin{cases}
        1, & \mbox{if }\mathrm{p}\mbox{ is a \textit{feature}} \\
        0, & \mbox{otherwise},
    \end{cases}
    \label{equ:feature or not}
\end{equation}
And we represent weight vector $\mathcal{R}^{\mathcal{F}}$ that derived from the amount of feature following as:
\begin{equation}
	\label{equ:weight_vector}
    \mathcal{R}_{[\mathbf{n}_{w}]}^{\mathcal{F}} = \sum_{j=\beta*[\mathbf{n}_{w}]}^{\beta*([\mathbf{n}_{w}]+1)} \left( \sum_{i=1}^{\mathcal{H}} \nu(\mathcal{I}^{\mathcal{F}}_{ij}) \right), \quad \mathcal{R}^{\mathcal{F}} \in\mathbb{R}^{\mathcal{N}_{w}},
\end{equation}
Since free space and features are inversely related, we create an \textit{R}-\textit{ReFeree} ($\mathcal{R}$) as follows:
\begin{equation}
	\label{equ:r_referee}
    \mathcal{R} = \mathcal{R}^{\mathcal{F}} \times \frac{1}{\mathcal{R}^{f}}.
\end{equation}
Also, \textit{A}-\textit{ReFeree}($\mathcal{A}$) for the initial estimation only performs normalization to produce the final description, as follows:
\begin{equation}
	\label{equ:a_referee}
    \mathcal{A} =\frac{\mathcal{A}^{f}}{\mathcal{N}_{h} \times \mathcal{W}}.
\end{equation}

\noindent When configuring \textit{A-ReFeree} as shown in the \figref{fig:detailed}, we count free space up to the farthest element due to radar's ability to penetrate particles.
% ==============================================================================================
\vspace{-0.3cm}
\begin{figure}[h]
	\centering
	\def\width{0.49\textwidth}%
    {%
        \includegraphics[clip, trim= 50 50 20 90, width=\width]{figs/freespace/freespace.pdf}
    }
        \vspace{-0.5cm}
        \caption{\textit{R-ReFeree} checks the free space for all rays, while \textit{A-ReFeree} calculates the free space up to a maximum feature distance.}	
\vspace{-0.2cm}
\label{fig:detailed}
\end{figure}
% ==============================================================================================

\noindent \bl{Although \textit{A-ReFeree} shows comparable performance to existing methods in loop detection \cite{choi2024referee} because it is a rotational variance descriptor, we use \textit{R-ReFeree} for place recognition.
% "A-ReFeree가 성능은 괜찮지만, rotational invariance가 없다" 는 내용?
Additionally, similar to what will be discussed in the next subsection, it does not demonstrate real-time performance.}
% 바로 위에 문장도 이상함
% "추가적으로 choi2024referee는 없지만 우리는 real-time performance를 달성했다" 는 내용?
% a-referee는 rotational invariance하지 않고, semi-metric 정보를 사용하여 reverse loop를 detection하더라도 real-time이 될 수 없다.

% ==============================================================================================
% \begin{figure}[t]
% 	\centering
% 	\def\width{0.49\textwidth}%
%     {%
%         \includegraphics[clip, trim= 170 130 150 100, width=\width]{figs/referee_compare/referee_compare.pdf}
%     }
%     \vspace{-0.7cm}
%     \caption{The 3D matching graph for \textit{R-ReFeree} and \textit{A-ReFeree} when the F1 score is maximized in the \textit{DCC} sequence of the \textit{Mulran} dataset.
%              Despite the presence of lane-level lateral variations, \textit{R-ReFeree} can identify a reverse loop, whereas \textit{A-ReFeree} fails to identify any.}
%     \vspace{-0.7cm}
%     \label{fig:referee_compare}
% \end{figure}
% ==============================================================================================

\subsubsection{Place Recognition}
We create the \textit{R-ReFeree} and recognize revisited places to correct accumulated pose errors. 
We construct a KD-Tree from the candidates to facilitate faster searching, and the distance between the query \textit{R}-\textit{ReFeree} $\mathcal{R}^q$ and the candidate \textit{R}-\textit{ReFeree} $\mathcal{R}^c$ is calculated using the L2-norm as follows:
\begin{equation}
    \sigma(\mathcal{R}^q, \mathcal{R}^c) = {||\mathcal{R}^q - \mathcal{R}^c||} .
    \label{equation:initial_index}
\end{equation}


\subsubsection{Initial Guess Estimation}
We can recognize revisited places through the \textit{R}-\textit{ReFeree}, and obtain the initial guess of the two places through the \textit{A}-\textit{ReFeree}.
Due to \hl{the rotational equivalence} and semi-metric information of the \textit{A}-\textit{ReFeree}, shifting candidates implies that the index of the closest distance represents $\hat{n}$ as a 1-DoF heading following:
\begin{equation}
    \hat{n} = \argmin\limits_{n \in [\mathbf{n}_{h}]}({||\mathcal{A}^q - \mathcal{A}}^{c}_{n}||) .
    \label{equation:initial_index}
\end{equation}

\subsubsection{Pose Graph Optimization}
% We identify revisited places through the \textit{R}-\textit{ReFeree} and also estimate the initial guess between these revisited places via \textit{A}-\textit{ReFeree}.
We require a registration process to correct errors \hl{in the accumulated map using odometry.}
Therefore, we adopt Nano-GICP \cite{chen2022direct}, which combines the fast speed of Fast-GICP \cite{koide2021voxelized} and the efficient construction of KD-Tree using the open-source library NanoFLANN \cite{blanco2014nanoflann}, not only for registration but also for onboard computing. 
First, we convert the estimated initial guess into a rotation matrix at loop $\mathcal{L}$:
\begin{equation}
 T^{\mathcal{L}}_{k} = \begin{bmatrix}
                  cos\left( \hat{n} \times \frac{360}{\mathcal{N}_{h}} \right) & -sin\left( \hat{n} \times \frac{360}{\mathcal{N}_{h}} \right) \\ 
                  sin\left( \hat{n} \times \frac{360}{\mathcal{N}_{h}} \right) &  cos\left( \hat{n} \times \frac{360}{\mathcal{N}_{h}} \right)
              \end{bmatrix} .	
\end{equation}
Second, we perform scan-to-scan matching between the source point $\mathcal{P}^{s}_{k}$ and the target point $\mathcal{P}^{t}_{k}$ to compute the optimal relative transform.
Finally, we obtain the optimal relative transformation.
However, even if detected and current places are in similar positions, mismatches in registration can introduce errors into the map.
Therefore, we progress a geometry verification process by calculating the fitness score through the \ac{ICP} result, which enables us to validate the accurate loop once more.
As pose graph $\mathbf{X}$ from radar odometry \cite{burnett_ral21} contains its accumulated errors due to sensor measurement, so loop closing is essential to build a consistent map.
The pose graph optimization of the map is represented as:
\begin{equation}
\begin{aligned}
\hat{\mathbf{X}}=\underset{\mathbf{X}}{\operatorname{argmin}} & \sum \varphi(\mathbf{X}) .
\end{aligned}
\end{equation}
Also, pose graph optimization fuction $\varphi(\cdot)$ is defined as:
\begin{equation}
\begin{aligned}
\varphi(\mathbf{X})= & \sum_t\left\|f\left(\mathbf{x}_t, \mathbf{x}_{t+1}\right)- \zeta({\mathbf{z}}_{t}, {\mathbf{z}}_{t+1})\right\|_{\sum_t}^2 \\
& +\sum_{\langle s, t \rangle \in \mathbb{L}} \left\|f\left(\mathbf{x}_s, \mathbf{x}_t\right)-\xi(\mathcal{P}^{s}_{k},\mathcal{P}^{t}_{k}) \right\|_{\sum_{s, t}}^2,
\end{aligned}
\end{equation}
where $f(\cdot, \cdot)$ is 6-DoF relative pose estimator, $\zeta(\cdot, \cdot)$ is radar odometry estimator with features $z_t$ that contain timestamp, $\xi(\cdot, \cdot)$ is pose aligner between $\mathcal{P}^{t}_{k}$ and $\mathcal{P}^{s}_{k}$ captured in $\mathcal{L} \in \mathbb{L}$. 
